Enhanced and Efficient Extraction of Uranyl Ions from Aqueous Waste through Graphene/CNT-PAMAM Nanocomposites

The increasing threat of uranium contamination to environmental and human health due to its radiotoxicity demands the development of novel and efficient adsorbents for remediation. In this study, we investigated the potential of poly(amidoamine) (PAMAM) dendrimers of generations 1 to 4 (G1 - G4) functionalized with graphene and carbon nanotubes (CNTs) as adsorbents for uranyl ion removal from aqueous solutions. By combining atomistic molecular dynamics (MD) simulations with experimental validation, we examined the influence of pH, uranyl ion concentration, and dendrimer generation on adsorption behavior. Our study revealed that uranyl ion adsorption is greater when PAMAM is grafted onto graphene/CNT than pristine PAMAM. However, PAMAM-grafted CNTs exhibit superior adsorption capacity at specific uranyl concentrations due to their curvature and abundant accessible binding sites. Higher-generation PAMAM dendrimers grafted onto graphene/CNTs exhibit greater adsorption capacity due to the increased availability of binding sites, which is consistent with experimental observations. The adsorption capability of uranyl ions in all four generations of the PAMAM dendrimer increased as the concentration of uranyl ions increased. Adsorption capacity increases with increasing uranyl ion concentration, and adsorption occurs on both PAMAM and graphene/CNT surfaces, with saturation observed at higher concentrations. This study provides insights into the adsorption mechanisms and highlights the potential of PAMAM-based nanocomposites for efficient uranyl ion extraction and environmental remediation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

